Automatic Extraction of Disease Risk Factors from Medical Publications

We present a novel approach to automating the identification of risk factors for diseases from medical literature, leveraging pre-trained models in the bio-medical domain, while tuning them for the specific task. Faced with the challenges of the diverse and unstructured nature of medical articles, our study introduces a multi-step system to first identify relevant articles, then classify them based on the presence of risk factor discussions and, finally, extract specific risk factor information for a disease through a question-answering model. Our contributions include the development of a comprehensive pipeline for the automated extraction of risk factors and the compilation of several datasets, which can serve as valuable resources for further research in this area. These datasets encompass a wide range of diseases, as well as their associated risk factors, meticulously identified and validated through a fine-grained evaluation scheme. We conducted both automatic and thorough manual evaluation, demonstrating encouraging results. We also highlight the importance of improving models and expanding dataset comprehensiveness to keep pace with the rapidly evolving field of medical research.

==> chapters/8-limitations.tex <==
\section{Limitations}
\label{sec:limitations}

Our study, while contributing valuable insights into the automation of risk factor identification from medical publications, is subject to several limitations that merit discussion.

One of the primary limitations is the challenge of accurately distinguishing risk factors specifically associated with the disease in question (mark 1) from valid risk factors that are not directly related to the disease under investigation (mark 2). While our models demonstrated a high capacity for identifying potential risk factors, the precision in contextualizing these factors to specific diseases varied. This aspect highlights a critical area for future research, emphasizing the need for enhanced specificity in the models to improve their utility in targeted medical research and practice.

Moreover, the study's reliance on free-text medical articles introduces variability in the data quality and representation. The unstructured nature of these texts and the diversity in how risk factors are described pose significant challenges for both the binary classification and question-answering models. Efforts to standardize data representation and improve model robustness against such variability are essential steps forward.

%Another limitation is the manual component of the dataset annotation process, particularly for the question-answering model. Despite leveraging medical students' expertise, the subjective nature of manual annotations can introduce biases and inconsistencies. Developing more sophisticated automated annotation tools or incorporating expert review mechanisms could help mitigate this issue.

The datasets used in this study, while extensive, are not exhaustive. The landscape of medical research is continuously evolving, with new findings emerging regularly. The datasets, therefore, represent a snapshot in time, and ongoing efforts to update and expand these resources are necessary to maintain their relevance and utility.

Finally, the study's scope was constrained by the computational resources available. Future work could explore more complex models or ensemble approaches that might offer improved accuracy but require more substantial computational power.

Despite these limitations, this study represents a significant step toward automating the identification of disease risk factors from medical literature. Acknowledging and addressing these limitations in future research will be crucial for advancing the field and enhancing the practical applicability of these technologies in healthcare.


==> chapters/9-closing-remarks.tex <==
\section{Closing Remarks}
\label{sec:closing-remarks}

The automation of disease risk factor identification from medical literature presents an exciting frontier in medical research and public health. By leveraging NLP technologies, we can uncover valuable insights more efficiently, ultimately contributing to preventive medicine and patient care. We look forward to the continued exploration of this field and the potential impacts of further advancements.
